ATT3D: Amortized Text-to-3D Object Synthesis

Text-to-3D modelling has seen exciting progress by combining generative text-to-image models with image-to-3D methods like Neural Radiance Fields. DreamFusion recently achieved high-quality results but requires a lengthy, per-prompt optimization to create 3D objects. To address this, we amortize optimization over text prompts by training on many prompts simultaneously with a unified model, instead of separately. With this, we share computation across a prompt set, training in less time than per-prompt optimization. Our framework - Amortized text-to-3D (ATT3D) - enables knowledge-sharing between prompts to generalize to unseen setups and smooth interpolations between text for novel assets and simple animations.

==> sections/intro.tex <==
%%%%%%%%% BODY TEXT
\vspace{-0.005\textheight}
\section{Introduction}\label{sec:intro}
\vspace{-0.005\textheight}
    %Topic: What are we trying do?
    %Topic: Why is it relevant?
    % Text-to-3D modeling has the potential to revolutionize real-time interactive 3D applications.
    % However, current methods suffer from high computational demands and produce suboptimal results.
    % One recent method, DreamFusion~\citep{poole2022dreamfusion}, achieves high-resolution detail but requires a lengthy, per-text-prompt optimization process and might create objects with unrealistic geometry (Fig. 9, row 4 ~\citep{poole2022dreamfusion}).
    % This work alleviates these issues with an amortized optimization procedure over text prompts, allowing us to bypass the expensive training procedure and immediately generate novel 3D objects, often helping with unrealistic geometries.
    
    Text-to-3D modeling has the potential to revolutionize real-time interactive 3D applications.
    However, current methods suffer from high computational demands and sub-optimal results.  
    DreamFusion~\citep{poole2022dreamfusion} and Magic3D~\citep{lin2022magic3d} recently achieved high-resolution detail but rely on a time-consuming optimization process for each text prompt.
    %This can lead to unrealistic geometry in generated objects (Fig. 9, row 4 ~\citep{poole2022dreamfusion}).
    We propose an amortized optimization approach to bypass the costly training, generate high-quality 3D objects, and interpolate between them.
    
    Our method learns a direct mapping from text prompts to Neural Radiance Fields (NeRFs)~\citep{mildenhall2021nerf} representing 3D scenes consistent with the text.
    With a new prompt, our method can cheaply produce an accurate NeRF model without requiring access to the large diffusion model or further optimization.
    To achieve this, we amortize the DreamFusion optimization over text prompts, vastly reducing the cost compared to independent text prompt training.
    We finetune our model with a small budget to match (or exceed) the quality of the single-prompt setting.

    \input{sections/interp_figure.tex}
    
    %Topic: Why is this hard?
    % However, classical methods designing models by hand with tools \Jon{cite} requires time and expertise.
    % Recent automatic methods of \Jon{cite Pre-dreamfusion} suffered from a lack of quality.
    % Most recently, Dreamfusion \Jon{cite} saw a leap in quality, but they suffered from:
    % (a) expensive training per prompt.
    % (b) visual artifacts from overfitting a single prompts samples.
    % DreamFusion uses an expensive per-prompt training designed to \emph{overfit} a single object-prompt pair.
    % The originally proposed NeRF architecture contains few parameters and does not have the required capacity to generate scenes corresponding to a diverse set of prompts.
    % The training objective itself has high variance and results in difficult training dynamics as the updates to the NeRF parameters affects the denoising model unpredictably \James{Can we make this sound less informal?}.
    % Through this observation, we liken the optimization procedure over multiple prompts to stochastic bi-level optimization.
    % Intuitively, this is similar to GAN training except the frozen diffusion model is not adversarial.
    DreamFusion's training objective \emph{overfits} a single object-prompt pair.
    The optimization pipeline is run from scratch each time, making large prompt sets prohibitively expensive.
    Extending this to a multi-prompt setting presents difficulties.
    % The training objective has high variance, as the rendering conditions are varied, while each batch element has a high memory cost.
    % The objective is poorly conditioned and approximates higher-order info with identity matrices.
    The NeRF's objective is specified by a denoising diffusion model (DDM) that changes during training akin to GANs~\citep{goodfellow2020generative, miyato2018spectral, brock2018large} and actor-critic models~\citep{pfau2016connecting}, while having high variance and poor conditioning.
    Also, standard NeRF architectures are designed to represent one scene and do not trivially extend to multiple scenes from diverse prompt sets.
    % Overfitting to a single prompt can introduce visual artifacts and prevents user interaction, such as interpolating between or combining different text prompts.
    
    % Topic: How do we solve it?
    We amortize the optimization procedure by reusing text embeddings to compute modulations to the NeRF, transforming the output to represent the text.
    We achieve this with a spatially oriented parameter grid modulated by a function of the text embeddings.
    Na\"ive implementations of this optimization problem are highly brittle.
    However, leveraging techniques from the bilevel optimization community, we stabilize training and scale our method. 
    
    % Topic: How do we verify that we have solved it? Experiments \& results + Theory
    %We assess our model's ability to (quickly and concisely) memorize and generalize to 3D scenes representing text prompts, on tasks from DreamFusion and that we setup for probing our model.
    
    \newcommand{\contributionSpaceShrink}{\vspace{-0.01\textheight}}  
    \subsection{Contributions}
        %\noindent
        We present a method to amortize the optimization of text-to-3D models, which allows us to:
        \contributionSpaceShrink
        \begin{itemize}
            \item Generalize to new prompts -- Fig.~\ref{fig:animals-compositional}.
            \contributionSpaceShrink
            \item Interpolate between prompts for user-guided asset generation and simplistic animations -- Fig.~\ref{fig:interpolation}.
            \contributionSpaceShrink
            \item Amortize over settings other than text prompts.
            \contributionSpaceShrink
            \item Reduce training time -- Fig.~\ref{fig:all_quantitative}.
            %\item Rapidly finetune on arbitrary prompts -- Fig.~\ref{fig:finetuning_qualitative}.
            % \contributionSpaceShrink
            % \item Reduce artifacts from overfitting prompts -- Fig.~\ref{fig:janus_reduction}.
        \end{itemize}
    
    % \subsection{Contribution Impact}
    %     In recent years, text-to-X generation-as-a-service has become very popular (HuggingFace, Stability, Runway, DALLE-2, etc…) and we are seeing a rise in text-to-X generation happening at a massive scale over many diverse sets of prompts being submitted daily.
    %     This has huge implications for the service providers in terms of energy and compute usage, as the total-cost-of-ownership for standard single prompt text-to-X generation systems scales linearly by the number of prompts.
    %     This is also an environmental concern… [cite studies of rainforests being burned down by GPUs].
    %     In our work, we show that we are able to significantly reduce costs over batches of prompts, showing sublinear scaling of text-to-X generation over prompts.
